On the Promises and Challenges of Multimodal Foundation Models for Geographical, Environmental, Agricultural, and Urban Planning Applications

The advent of large language models (LLMs) has heightened interest in their potential for multimodal applications that integrate language and vision. This paper explores the capabilities of GPT-4V in the realms of geography, environmental science, agriculture, and urban planning by evaluating its performance across a variety of tasks. Data sources comprise satellite imagery, aerial photos, ground-level images, field images, and public datasets. The model is evaluated on a series of tasks including geo-localization, textual data extraction from maps, remote sensing image classification, visual question answering, crop type identification, disease/pest/weed recognition, chicken behavior analysis, agricultural object counting, urban planning knowledge question answering, and plan generation. The results indicate the potential of GPT-4V in geo-localization, land cover classification, visual question answering, and basic image understanding. However, there are limitations in several tasks requiring fine-grained recognition and precise counting. While zero-shot learning shows promise, performance varies across problem domains and image complexities. The work provides novel insights into GPT-4V's capabilities and limitations for real-world geospatial, environmental, agricultural, and urban planning challenges. Further research should focus on augmenting the model's knowledge and reasoning for specialized domains through expanded training. Overall, the analysis demonstrates foundational multimodal intelligence, highlighting the potential of multimodal foundation models (FMs) to advance interdisciplinary applications at the nexus of computer vision and language.

==> statement.tex <==
\vspace{-0.5cm}
\section*{Statements and Declarations} 

\paragraph{Acknowledgements}
Dr. Gengchen Mai acknowledges the support from the University of Georgia's International Intellectual Property Alliance (IIPA) Seed Grant -- 'SSIF: A Deep Generative Model for Remote Sensing Image Spatial-Spectral Super-Resolution for Precision Agriculture'. Dr. Lilong Chai acknowledges the support from USDA-NIFA AFRI (2023-68008-39853). Dr. Changying Li acknowledges funding support from USDA-NIFA Data Science for Food and Agricultural Systems (2023-67021-40646).

\paragraph{Competing Interests}
The author declares that he/she has no financial or non-financial interests that are directly or indirectly related to the work submitted for publication.

\paragraph{Availability of data and material}
All data we used for publically available datasets.

\paragraph{Funding}
University of Georgia's International Intellectual Property Alliance (IIPA) Seed Grant -- 'SSIF: A Deep Generative Model for Remote Sensing Image Spatial-Spectral Super-Resolution for Precision Agriculture'; USDA-NIFA AFRI (2023-68008-39853); USDA-NIFA DSFAS (2023-67021-40646).

\paragraph{Authors' contributions}
Chenjiao Tan and Dr. Changying Li are responsible for all plant disease, weed recognition, and phenotyping experiments. Qian Cao is responsible for image geo-localization and urban planning tasks. Yiwei Li and Zhdengliang Liu are responsible for the introduction and related work section writing. Jielu Zhang is responsible for experiments on fine-grain crop classification task, remote sensing visual question answering task, and air quality evaluation task. Xiao Yang and Dr. Lilong Chai are responsible for poultry science experiments. Nemin Wu is responsible for historical map text extraction and localization tasks. Hao Yang is responsible for the crop nutrient deficiency detection task. Dr. Tao Yang contributed to paragraph writing for the GPT-4V's applications on Urban Planning tasks. Dr. Xinyue Ye, Dr. Ninghao Liu, Dr. Lan Mu, Dr. Tianming Liu contributed to the overall paper writing and revision. Dr. Gengchen Mai is responsible for the overall project organization, task assignment, paper writing, revision, and submission.

% \paragraph{Financial interests}
% None

% \paragraph{Non-financial interests}
% None
